Real-time optimal control via Deep Neural Networks: study on landing problems

Recent research on deep learning, a set of machine learning techniques able to learn deep architectures, has shown how robotic perception and action greatly benefits from these techniques. In terms of spacecraft navigation and control system, this suggests that deep architectures may be considered now to drive all or part of the on-board decision making system. In this paper this claim is investigated in more detail training deep artificial neural networks to represent the optimal control action during a pinpoint landing, assuming perfect state information. It is found to be possible to train deep networks for this purpose and that the resulting landings, driven by the trained networks, are close to simulated optimal ones. These results allow for the design of an on-board real time optimal control system able to cope with large sets of possible initial states while still producing an optimal response.

==> quadrotor.tex <==
\begin{figure}[t!]
\centering
\begin{tikzpicture}
    % Lets draw the inertial reference system
    \draw[thin,->] (0,0) -- (3,0) node[anchor=north west] {$\hat{\mathbf i}_x$};
    \draw[thin,->] (0,0) -- (0,3) node[anchor=south east] {$\hat{\mathbf i}_y$};
    
    % And now, lets draw the rocket
    \def\rocketrot{30}
    \begin{scope}[rotate=-\rocketrot]
        % Coordinates of the COM
        \def\x{0}
        \def\y{0}
        % Rocket Shape: width and height
        \def\w{2}
        \def\h{0.2}

        % Coordinates of the rocket body
        \coordinate (LL) at (\x - \w / 2, \y - \h / 2);
        \coordinate (LR) at (\x + \w / 2, \y - \h / 2);
        \coordinate (UL) at (\x - \w / 2, \y + \h / 2);
        \coordinate (UR) at (\x + \w / 2, \y + \h / 2);
        \coordinate (NOSE) at (\x, \y + \h / 2 + \h / 6);
        % Coordinates for the thrust
        \coordinate (Torigin) at (\x,\y - \h / 2 - \h / 12);
        \coordinate (Tvect) at (1.5,1.5);
        % Coordinates for the nozzle
        \coordinate (Norigin) at (\x, \y - \h / 2);
        \coordinate (NL) at (\x - \w / 4, \y - \h / 2 - \h / 12);
        \coordinate (NR) at (\x + \w / 4, \y - \h / 2 - \h / 12);
        
        \coordinate (O) at (\x, \y + \h / 2 + \h / 3);
        
        % Lets draw the body reference system
        %\draw[thin,->] (O) -- ($(O) + (1,0)$) node[anchor=north west] {$\hat{\mathbf i}_\tau$};
        \draw[thin,->] (O) -- ($(O) + (0,1)$) node[anchor=south west] {$\hat{\mathbf i}_\theta$};
        
        % The COM
        % \fill[fill=black!70!white](0,0) -- (\w/2, 0) arc (0:90:\w/2);
        %\fill[fill=black!70!white](0,0) -- (-\w/2, 0) arc (180:270:\w/2);
        %\draw (0,0) circle (\w/2);
        
        % The rocked body
        \draw[] (LL) -- (UL) -- (NOSE) -- (UR) -- (LR) -- (LL);
        
        % The nozzle
        %\draw[] (Norigin) -- (NL) -- (NR) -- (Norigin);
        
        % The symmetry axis
        \draw[thin, dashed] (0,-2) -- (0,1.7);
        
        % The thrust
        %\draw [thick, ->] (Torigin) -- ($(Torigin) + (Tvect)$) %node[midway,below] {$c_1 u \hat{\mathbf t}$};
    \end{scope}
    
    %gravity
    \draw [thick, ->] (0,0) -- (0,-1) node[midway,right] {$\mathbf g$};
    
    % the angle theta
    \draw (0,0) ++(90:.8) arc (90:90-\rocketrot:.8) node[midway,above] {$\theta$};
    
\end{tikzpicture}
\caption{Reaction wheel spacecraft model}
\end{figure}

==> simplepicture.tex <==
\begin{figure}[t!]
\centering
\begin{tikzpicture}
    % Lets draw the inertial reference system
    \draw[thin,->] (0,0) -- (3,0) node[anchor=north west] {$\hat{\mathbf i}_x$};
    \draw[thin,->] (0,0) -- (0,3) node[anchor=south east] {$\hat{\mathbf i}_y$};
    
    % And now, lets draw the rocket
    \def\rocketrot{30}
    \begin{scope}[rotate=-\rocketrot]
        % Coordinates of the COM
        \def\x{0}
        \def\y{0}
        % Rocket Shape: width and height
        \def\w{2}
        \def\h{2}

        % Coordinates of the rocket body
        \coordinate (LL) at (\x - \w / 2, \y - \h / 2);
        \coordinate (LR) at (\x + \w / 2, \y - \h / 2);
        \coordinate (UL) at (\x - \w / 2, \y + \h / 2);
        \coordinate (UR) at (\x + \w / 2, \y + \h / 2);
        \coordinate (NOSE) at (\x, \y + \h / 2 + \h / 6);
        % Coordinates for the thrust
        \coordinate (Torigin) at (\x,\y - \h / 2 - \h / 12);
        \coordinate (Tvect) at (1.5,1.5);
        % Coordinates for the nozzle
        \coordinate (Norigin) at (\x, \y - \h / 2);
        \coordinate (NL) at (\x - \w / 4, \y - \h / 2 - \h / 12);
        \coordinate (NR) at (\x + \w / 4, \y - \h / 2 - \h / 12);
        
        \coordinate (O) at (\x, \y + \h / 2 + \h / 3);
        
        % Lets draw the body reference system
        %\draw[thin,->] (O) -- ($(O) + (1,0)$) node[anchor=north west] {$\hat{\mathbf i}_\tau$};
        \draw[thin,->] (O) -- ($(O) + (0,1)$) node[anchor=south west] {$\hat{\mathbf i}_\theta$};
        
        % The COM
        % \fill[fill=black!70!white](0,0) -- (\w/2, 0) arc (0:90:\w/2);
        %\fill[fill=black!70!white](0,0) -- (-\w/2, 0) arc (180:270:\w/2);
        %\draw (0,0) circle (\w/2);
        
        % The rocked body
        \draw[] (LL) -- (UL) -- (NOSE) -- (UR) -- (LR) -- (LL);
        
        % The nozzle
        \draw[] (Norigin) -- (NL) -- (NR) -- (Norigin);
        
        % The symmetry axis
        \draw[thin, dashed] (0,-2) -- (0,1.7);
        
        % The thrust
        %\draw [thick, ->] (Torigin) -- ($(Torigin) + (Tvect)$) %node[midway,below] {$c_1 u \hat{\mathbf t}$};
    \end{scope}
    
    %gravity
    \draw [thick, ->] (0,0) -- (0,-1) node[midway,right] {$\mathbf g$};
    
    % the angle theta
    \draw (0,0) ++(90:.8) arc (90:90-\rocketrot:.8) node[midway,above] {$\theta$};
    
\end{tikzpicture}
\caption{Reaction wheel spacecraft model}
\end{figure}
